A Turning Point for Verified Spectre Sandboxing

Spectre attacks enable an attacker to access restricted data in an application's memory. Both the academic community and industry veterans have developed several mitigations to block Spectre attacks, but to date, very few have been formally vetted; most are "best effort" strategies. Formal guarantees are particularly crucial for protecting isolated environments like sandboxing against Spectre attacks. In such environments, a subtle flaw in the mitigation would allow untrusted code to break out of the sandbox and access trusted memory regions. In our work, we develop principled foundations to build isolated environments resistant against Spectre attacks. We propose a formal framework for reasoning about sandbox execution and Spectre attacks. We formalize properties that sound mitigation strategies must fulfill and we show how various existing mitigations satisfy (or fail to satisfy!) these properties.

==> rref.tex <==
%
%
%
%
%
%
%
%

\makeatletter%
%
%
\eh@everypar{\eh@prepar\the\expandafter\eh@privatepar\eh@postpar}%
\newcount\ruleref@parcount%
\ruleref@parcount0%
\PushPreHook{par}{\ruleref@newpar}%
\def\ruleref@newpar{%
  \global\advance\ruleref@parcount by 1%
  \edef\ruleref@lastpar{par.\the\ruleref@parcount}%
  \expandafter\Hy@raisedlink\expandafter{\expandafter\hypertarget\expandafter{\ruleref@lastpar}{}}%
}%
\let\ruleref@DefTirName=\DefTirName%
\let\ruleref@LabTirName=\LabTirName%
\def\ruleref@aux@namedef#1#2{%
  \global\@namedef{ruleref@defined@#1}{#2}%
  \immediate\write\@auxout{\global\string\@namedef{#1}{#2}}%
}%
\def\IgnoreUnusedRule#1{%
  \expandafter\gdef\csname ruleref@unusedrule@#1\endcsname{}%
}%
\def\DefTirName#1{{%
  \ifcsname ruleref@rulecount@#1\endcsname%
    \expandafter\expandafter\expandafter\count@\csname ruleref@rulecount@#1\endcsname%
    \advance\count@ by 1%
    \expandafter\xdef\csname ruleref@rulecount@#1\endcsname{\the\count@}%
  \else%
    \expandafter\gdef\csname ruleref@rulecount@#1\endcsname{0}%
    \ruleref@aux@namedef{ruleref@ruledefn@#1}{}%
  \fi%
  \edef\theusecmd{ruleref@use@#1@\csname ruleref@rulecount@#1\endcsname}%
  \Hy@raisedlink{\hypertarget{rule.def.#1.\csname ruleref@rulecount@#1\endcsname}{}}%
  \ifcsname\theusecmd\endcsname%
    \expandafter\hyperlink\expandafter{%
      \csname\theusecmd\endcsname%
    }{%
      \ruleref@DefTirName{#1}%
    }%
  \else%
    \ifcsname ruleref@unusedrule@#1\endcsname%
    \else%
      \@latex@warning{Could not find use/explanation for #1 definition%
        \csname ruleref@rulecount@#1\endcsname. Rerun.}%
    \fi%
    \ruleref@DefTirName{#1}%
  \fi%
}}%
\def\LabTirName#1{{%
  \ifcsname ruleref@unusedrule@#1\endcsname%
    \@latex@warning{Used ``unused'' rule #1! Rerun}.%
  \fi%
  \ifcsname ruleref@rulecount@#1\endcsname%
    \edef\therulecount{\csname ruleref@rulecount@#1\endcsname}%
  \else%
    \edef\therulecount{0}%
    \ifcsname ruleref@ruledefn@#1\endcsname%
    \else%
      \@latex@warning{Could not find rule definition for #1. Rerun.}%
    \fi%
  \fi%
  \edef\theusecmd{ruleref@use@#1@\therulecount}%
  \ifcsname ruleref@defined@\theusecmd\endcsname%
  \else%
    \ifcsname\theusecmd\endcsname%
      \ifnum\pdfstrcmp{\csname\theusecmd\endcsname}{par.\the\ruleref@parcount}=0%
      \else%
        \@latex@warning{Reference changed for #1 definition%
          \therulecount. Rerun.}%
      \fi%
    \else%
    \fi%
    \ruleref@aux@namedef{\theusecmd}{par.\the\ruleref@parcount}%
  \fi%
  \hyperlink{rule.def.#1.\therulecount}{\ruleref@LabTirName{#1}}%
}}%
\makeatother%
\newcommand{\rref}[1]{\LabTirName{#1}}%

